Understanding Semantics from Speech Through Pre-training

End-to-end Spoken Language Understanding (SLU) is proposed to infer the semantic meaning directly from audio features without intermediate text representation. Although the acoustic model component of an end-to-end SLU system can be pre-trained with Automatic Speech Recognition (ASR) targets, the SLU component can only learn semantic features from limited task-specific training data. In this paper, for the first time we propose to do large-scale unsupervised pre-training for the SLU component of an end-to-end SLU system, so that the SLU component may preserve semantic features from massive unlabeled audio data. As the output of the acoustic model component, i.e. phoneme posterior sequences, has much different characteristic from text sequences, we propose a novel pre-training model called BERT-PLM, which stands for Bidirectional Encoder Representations from Transformers through Permutation Language Modeling. BERT-PLM trains the SLU component on unlabeled data through a regression objective equivalent to the partial permutation language modeling objective, while leverages full bi-directional context information with BERT networks. The experiment results show that our approach out-perform the state-of-the-art end-to-end systems with over 12.5% error reduction.

==> motivation.tex <==


So we can change the calculation order as follows.
\begin{itemize}
\item 
\item Given the sampled context, we then predict all the possible $x_{z_t}$ from the rest of the sequence as targets, which forms the target subsequence $\overline{\mathbf{x}}$.
\end{itemize}
W


The calculation of $\log p_\theta(\overline{\mathbf{x}}|\hat{\mathbf{x}})$ can be easily done in parallel, which will be discussed below in detail.




So if, 



Therefore, the phoneme posterior sequence $\bm{H}^{phoneme}$ generated from some piece of audio has the following characteristics.




In this section, we firstly introduce the whole architecture of the phoneme pre-training based end-to-end spoken language understanding. Then we introduce the details of the proposed Bidirectional Encoder Representations from Transformers based on Permutation Language model (BERT-PL). Finally, we prove that the proposed BERT-PLM is equal to XLNET.


However, the pre-trained ELMo structures may not be directly used in the downstream tasks as 
Unsupervised NLP pre-training approaches, such as , BERT\citep{Devlin:2019}, ERNIE\citep{sun2019ernie}, GPT and GPT2\citep{Radford:2018} as well as 
This saves hundreds and thousands GPU/TPU hours for anyone in NLP research community to build well-performed models.

According to the training objectives, language models can be divided into to two camps: the AE(Auto-Encoding) and AR(Auto-Regressive). 
AE language modeling based pre-training approaches including BERT\citep{Devlin:2019} \& ERNIE\citep{sun2019ernie}, try to reconstruct the masked input $\widehat{x}$ based on the corrupted input(context) $\overline{x}$:
\begin{equation}
\label{bert_equation}
    \max \log p_\theta(\overline{\mathbf{x}}|\widehat{\mathbf{x}}) \approx \sum_{t=1}^{T}{m_t\log p_\theta(x_t|\widehat{\mathbf{x}})}
\end{equation}
where $m_t$ is an indicator equaling 1 when $x_t$ is masked otherwise 0. The difference is BERT randomly select tokens to be masked while ERNIE randomly select consecutive input tokens to be masked. 

Conventional AR language modeling based approaches like ELMo\citep{peters2018deep}, GPT \& GPT2\citep{Radford:2018} perform pre-training by maximizing the likelihood under the forward auto-regressive factorization:
\begin{equation}
\label{ar_equation}
    \max \log p_\theta(\mathbf{x}) = \sum_{t=1}^{T}{\log p_\theta(x_t|\mathbf{x}_{<t})}
\end{equation}

Analytically, we compare these two different language models:

\noindent \textbf{AR Language Modeling based Pre-training}
\begin{description}
  \item[$\bullet$ Pros] Consistency between the pre-training phase and the fine-tuning phase as no artificial [MASK] token is involved. It doesn't have to suffer from the corrupted input as AE models do. 
  \item[$\bullet$ Cons] The objective of factorization probability is conditioned on the contextual information from single direction which means limited information can be obtained.
\end{description}

\noindent \textbf{AE Language Modeling based Pre-traininig}
\begin{description}
  \item[$\bullet$ Pros] Access to the contextual information from both sides. BERT objective allows the model to be pretrained to better capture bidirectional context.
  \item[$\bullet$ Cons] Inconsistency between the pre-traininig phase and fine-tuning phase as the introduction of the artificial [MASK] token. What's more, as shown in Eq.\ref{bert_equation}, the $\approx$ symbol is used as BERT factorizes the joint conditional probability $p(\overline{x}|\widehat{x})$ assuming that all masked tokens are separately reconstructed.
\end{description}

With the pros and cons in existing pre-training approaches, XLNET was proposed to leverage the best of both AE and AR language models while avoiding their limitations.
Instead of calculating a fixed forward or backward factorization probability, XLNET maximizes the expected log likelihood of a sequence with respect to all possible permutations of the factorization order. While the permutation language modeling objective has several benefits, there exists a challenging optimization problem due to the permutation and causes slow convergence, XLNET choose to predict the last few tokens in a factorization order calling partial prediction:
% \begin{equation}
%     \label{XLNET_equation}
%     \max \mathbb{E}_{z\sim Z_T} \left[\log p_\theta (x_{z>c}|x_{z_{\leq{c}}}) \right]
% \end{equation}

\begin{equation}\label{XLNET_equation}
     \max \mathbb{E}_{\mathbf{z}\sim Z_T}\big{[}\log p(\mathbf{x}_{\mathbf{z}_{>c}}|\mathbf{x}_{\mathbf{z} \leq c})\big{]}
\end{equation}
where $Z_T$ denotes all possible permutations of a length-$T$ sequence$[1,2,...,T]$, $z_t$ and $\mathbf{z}_{<t}$ denote the $t$-th element and  the first $t$-1 elements of a permutation $\mathbf{z}\in Z_T$, respectively. The objective only permutes the factorization order rather than the original sequence order. 
As XLNET is a generalized AR model, naturally it doesn't suffer from the corruption input as BERT do. 




The Figure~\ref{fig:whole_arc} shows the whole architecture of our proposed phoneme pre-training based BERT-PLM will be introduced in next subsection. Finally, we use the limited SLU labeled audio data to fine-tune the pre-trained model. In addition, to accelerate the convergence, we build a multi-task to optimize the mask language model loss and classification loss.




\subsection{BERT-PLM}
XLNET propose a two-stream self-attention architecture for the proposed partial prediction of permutation language modeling training objective as standard Transformer parameterization may not work while we give theoretical proof that the partial prediction of permutation language modeling can be implemented in a BERT way by randomly sampling number of tokens to be masked as well as remove the [MASK] token by attention mask.
Formally, we give the definition of BERT-PLM:
\begin{equation}
    \label{BERTPL_equation}
    \max \mathbb{E}_{|\overline{\mathbf{x}}|\sim [1, T-c]} \left[\log p (\overline{\mathbf{x}}|\hat{\mathbf{x}}) \right]
\end{equation}
where $|\overline{\mathbf{x}}|$ denotes number of tokens(or frames of phonemes in SLU tasks pre-training) chosen to be masked, the expectation in Eq.\ref{BERTPL_equation} means the number of masks is subject to a uniform distribution $[1, T-c]$. We randomly select the number of masks during pre-training. As for the corrupted input $\hat{\mathbf{x}}$, we do not involve the [MASK] symbol both during the pre-training phase and the fine-tuning phase, instead we use attention mask to mask the $K,Q,V$ during self-attention calculation corresponding to the masked input.
\subsection{Theoretical Proof}
We claim the proposed BERT-PLM is equivalent to the XLNET in masking mechanism and permutation language model. The partial permutation language model in XLNET is calculated by Eq. \ref{XLNET_equation}.
% \begin{Eq.*}
    
%     \begin{aligned}
%      \mathbb{E}_{\mathbf{z}\sim Z_T}\big{[}\log p(\mathbf{x}_{\mathbf{z}_{>c}}|\mathbf{x}_{\mathbf{z} \leq c})\big{]}
%     \end{aligned}
%     \eqno{(1)}
% \end{Eq.*}
% \begin{Eq.*}
%     \begin{aligned}
%      p(\mathbf{x}_{\mathbf{z}_{>c}}|\mathbf{x}_{\mathbf{z} \leq c})=\sum_{t=c+1}^{|\mathbf{z}|}\log p(x_{z_t}|\mathbf{x}_{\mathbf{z}_{<t}})
%     \end{aligned}
%     \eqno{(2)}
% \end{Eq.*}

% \begin{Eq.}
%      p(\mathbf{x}_{\mathbf{z}_{>c}}|\mathbf{x}_{\mathbf{z} \leq c})=\sum_{t=c+1}^{|\mathbf{z}|}\log p(x_{z_t}|\mathbf{x}_{\mathbf{z}_{<t}})
% \end{Eq.}
% where $Z_T$ is the set of all possible permutations of the length-$T$ index sequence $[1,2,...,T]$. we use $z_t$ and $\mathbf{z}_{<t}$ to denote the $t$-th element and the first $t$-1 elements of a permutation $\mathbf{z}\in Z_T$.
The expectation of Eq. \ref{XLNET_equation} can be represented as:
% \begin{eqnarray}
%      \lefteqn{{}}
%      \nonumber \\
%      & & {}
% \end{eqnarray}

\begin{equation} \label{equ:equal}
\begin{aligned}
&\frac{\displaystyle\sum_{\mathbf{z}\in Z_T}\log p(\mathbf{x}_{\mathbf{z}_{>c}}|\mathbf{x}_{\mathbf{z} \leq c})}{T!}\\
&=\frac{\displaystyle\sum_{\mathbf{z}\in Z_T}\sum_{t=c+1}^{|\mathbf{z}|}\log p(x_{z_t}|\mathbf{x}_{\mathbf{z}_{<t}})}{T!} \\
&= \frac{\displaystyle\sum_{t=c+1}^{|\mathbf{z}|}\sum_{\mathbf{z}\in Z_T}\log p(x_{z_t}|\mathbf{x}_{\mathbf{z}_{<t}})}{T!}\\
&= \frac{\displaystyle\sum_{t=c+1}^{|\mathbf{z}|}\sum_{\mathbf{z}\in Z^*_T}\log p(x_{z_t}|\mathbf{x}_{\mathbf{z}_{<t}}) (T-t)!(t-1)!}{T!}\\
&=\frac{\displaystyle
\sum_{t=c+1}^{|\mathbf{z}|}
\sum_{i=1}^{\mathrm{C}^{T-t+1}_{T}}
\sum_{j=1}^{T-t+1}
\log p(x_j|\mathbf{\hat{x}}_i) (T-t)!(t-1)!(T-t+1)
}
{T!}\\
&=\sum_{t=c+1}^{|\mathbf{z}|}
\frac{
\sum_{i=1}^{\mathrm{C}^{T-t+1}_{T}}
\sum_{j=1}^{T-t+1}
\log p(x_j|\mathbf{\hat{x}}_i)
}
{
\frac{T!}{(T-t+1)!(t-1)!}
}\\
&=\sum_{t=c+1}^{|\mathbf{z}|}
\frac{
\sum_{i=1}^{\mathrm{C}^{T-t+1}_{T}}
\log p(\overline{\mathbf{x}}|\mathbf{\hat{x}}_i)
}
{\mathrm{C}_T^{T-t+1}}\\
&=\mathbb{E}_{|\overline{\mathbf{x}}|\sim [1, T-c]} \left[\log p (\overline{\mathbf{x}}|\hat{\mathbf{x}}) \right]
\end{aligned}
\end{equation}
where $Z_T$ denotes all possible permutation of a length-$T$ sequence. 
For a fixed three segments of a permutation $[x_1,x_2,...x_{t-1}],x_t,[x_{t+1},x_{t+2},...,x_T]$, the first part and last part has $(t-1)!$ and $(T-t)!$ permutation.
Thus, $Z_T^*$ denotes the unique permutations of a fixed three segments.
From the Eq.\ref{equ:equal}, we can see that the expectation of BERT-PLM is same with the expectation of XLNET.

%FSC
\begin{table} [h]
% table caption is above the table
\caption{The experiment result of the Google Speech Command dataset}
\label{tab:sc}       % Give a unique label
% For LaTeX tables use
\centering
\begin{tabular}{lc}
\hline\noalign{\smallskip}
Model & ACC \\
\noalign{\smallskip}\hline\noalign{\smallskip}
SOTA & $96.21\%$ \\
model/pret & $90.85\%$ \\
OPEN-GPT & $91.02\%$ \\
BERT & $91.34\%$ \\
ERNIE & $91.67\%$ \\
XLNET & $92.09\%$ \\
BERT-PLM & $92.11\%$ \\
\noalign{\smallskip}\hline
\end{tabular}
\end{table}








\section{Motivation}
\label{sec:motivation}
In information theory, there are some information loss after a signal passes a certain channel, and the information loss in previous channel cannot be recovered in subsequent steps.
Similarly, the traditional SLU pipeline also faces the problem of information loss. 
Especially the ASR errors, which can hardly be corrected by the following NLU models. 
Some end-to-end SLU methods, where the intermediate results of ASR are directly used in the following NLU model, are proposed to alleviate this problem.
However, noting that one kind of phoneme sequence is corresponded to several different kinds of text words, which means the text words would possess more information than textless phonemes because the text words are designed by human-beings to encode more knowledge.
While from another point of view, we observe that a language can be represented as either text word or textless phonemes.
Let's take Japanese for example, the hiragana and katakana are used in a mixed way with each other in Japanese(the katakana can be interpreted as one kind of phoneme sequence).

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.07]{figures/1.jpeg}
%     \caption{\begin{CJK}{UTF8}{min}
        
%     \end{CJK}}
%     \label{fig:doramon}
% \end{figure}



In extreme cases, a spoken language can be entirely represented by katakana.
As a result, we believe that there is no need to translate the audio to text words for people to understand an intent of spoken language.

Motivated by this phenomenon, we propose to use the phoneme posterior distribution to do the following NLU task among different intermediate feature of ASR.
And also the information loss from audio to phoneme posterior is less, which can be ignored.
The problem of pronunciation and environment noise can be greatly alleviated by using the phoneme posterior distribution.
To learn more semantic information, we try to conduct context-aware phoneme representation learning, which is called phoneme pre-training, from large-scale unlabeled audio data just as the pre-training models in text, such as BERT and XLNET.
Especially, it is hard to do pre-training on audio level and the pre-training on text is less benefitial because the information loss is serious in ASR.
Thus, the phoneme posterior is most suitable used in current end-to-end SLU architecture.



%Snips
\begin{table} [h]
% table caption is above the table
\caption{The experiment result of the snips dataset}
\label{tab:snips}       % Give a unique label
% For LaTeX tables use
\centering
\begin{tabular}{lcccc}
\hline\noalign{\smallskip}
Field&\multicolumn{2}{c}{Close Field}&\multicolumn{2}{c}{Far Field}\\
\noalign{\smallskip}\hline\noalign{\smallskip}
Model & Macro-F1 & Micro-F1 & Macro-F1 & Micro-F1  \\
\noalign{\smallskip}\hline\noalign{\smallskip}
SOTA & - & $92.00\%$ & - & $84.00\%$ \\
model/pret & $56.45\%$ & $59.04\%$ & $33.51\%$ & $38.01\%$ \\
OPEN-GPT & $64.86\%$ & $65.48\%$ & $45.16\%$ & $46.34\%$ \\
BERT & $66.12\%$ & $67.36\%$ & $46.32\%$ & $47.91\%$ \\
ERNIE & $66.08\%$ & $67.26\%$ & $47.76\%$ & $48.43\%$ \\
XLNET & $68.78\%$ & $69.31\%$ & $49.21\%$ & $50.31\%$ \\
BERT-PLM & $69.46\%$ & $70.36\%$ & $49.58\%$ & $51.93\%$ \\
\noalign{\smallskip}\hline
\end{tabular}
\end{table}



==> slot_result_table.tex <==
\begin{table}
	\centering
	\caption{\label{tab:lf_results} Slot result table.}
	\begin{tabular}{ll}
		\hline 
		\multicolumn{1}{l}{\textbf{Approach}} & 
	    \multicolumn{1}{c}{\textbf{F1}} \\ \hline \hline
		Seq2Seq & 28.0\%  \\
		SLOT Value & 50.0\%  \\ 
		+ Slot Encoder & 54.0\%   \\
		+ pointer Gate & 57.0\%  \\ 
		+ Global Encoder & 82.0\%  \\ 
		+ Segment Embedding & 82.5\%  \\ 
		+ Relative Position & 83.0\%  \\ 
		\hline
	\end{tabular}

\end{table}
